On the Linear Algebraic Structure of Distributed Word Representations

In this work, we leverage the linear algebraic structure of distributed word representations to automatically extend knowledge bases and allow a machine to learn new facts about the world. Our goal is to extract structured facts from corpora in a simpler manner, without applying classifiers or patterns, and using only the co-occurrence statistics of words. We demonstrate that the linear algebraic structure of word embeddings can be used to reduce data requirements for methods of learning facts. In particular, we demonstrate that words belonging to a common category, or pairs of words satisfying a certain relation, form a low-rank subspace in the projected space. We compute a basis for this low-rank subspace using singular value decomposition (SVD), then use this basis to discover new facts and to fit vectors for less frequent words which we do not yet have vectors for.

==> acknowledgements.tex <==
\chapter{Acknowledgements}

\begin{itemize}
\item David Kong

\item Billy Fang

\item math professors

\item Mimi Lee

\item Ming-Yee for help on Perl, processing the wikipedia corpus

\item Channing Huang for helping me configure emacs so it's pretty, for telling me about nohup so I could run code on the cluster

\item Prof. Arora

\item Yingyu Liang - for his code and analogies, for explaining GloVe code to me

\item Manna Christian Fellowship

\item Sola, Irene?

\end{itemize}


==> table-learn_new_facts-acc.tex <==
\begin{subtable}{.5\textwidth}\centering
\subcaption{$c=\texttt{classical\_composer}$}
\begin{tabular}{ | t | c |}\hline
word & projection\\ \hline
schumann & 0.841 \\
beethoven & 0.840 \\
stravinsky & 0.796 \\
liszt & 0.789 \\
schubert & 0.788 \\
\hline\end{tabular}
\end{subtable}\begin{subtable}{.5\textwidth}\centering\subcaption{$c=\texttt{sport}$}\begin{tabular}{ | t | c |}\hline
word & projection\\ \hline
biking & 0.881 \\
volleyball & 0.870 \\
skiing & 0.810 \\
softball & 0.809 \\
soccer & 0.801 \\
\hline\end{tabular}\end{subtable}\vspace{5ex}

\begin{subtable}{.5\textwidth}\centering\subcaption{$c=\texttt{university}$}\begin{tabular}{ | t | c |}\hline
word & projection\\ \hline
cambridge\_university & 0.897 \\
university\_of\_california & 0.889 \\
new\_york\_university & 0.868 \\
stanford\_university & 0.824 \\
yale\_university & 0.822 \\
\hline\end{tabular}\end{subtable}\vspace{5ex}\begin{subtable}{.5\textwidth}\centering\subcaption{$c=\texttt{basketball\_player}$}\begin{tabular}{ | t | c |}\hline
word & projection\\ \hline
dwyane\_wade & 0.788 \\
aren & 0.721 \\
kobe\_bryant & 0.715 \\
chris\_bosh & 0.712 \\
tim\_duncan & 0.708 \\
\hline\end{tabular}\end{subtable}

\begin{subtable}{.5\textwidth}\centering\subcaption{$c=\texttt{religion}$}\begin{tabular}{ | t | c |}\hline
word & projection\\ \hline
christianity & 0.899 \\
hinduism & 0.880 \\
taoism & 0.863 \\
buddhist & 0.846 \\
judaism & 0.830 \\
\hline\end{tabular}\end{subtable}\begin{subtable}{.5\textwidth}\centering\subcaption{$c=\texttt{tourist\_attraction}$}\begin{tabular}{ | t | c |}\hline
word & projection\\ \hline
metropolitan\_museum\_of\_art & 0.822 \\
museum\_of\_modern\_art & 0.813 \\
london & 0.764 \\
national\_gallery & 0.764 \\
tate\_gallery & 0.756 \\
\hline\end{tabular}\end{subtable}\vspace{5ex}

\begin{subtable}{.5\textwidth}\centering\subcaption{$c=\texttt{holiday}$}\begin{tabular}{ | t | c |}\hline
word & projection\\ \hline
diwali & 0.821 \\
christmas & 0.806 \\
passover & 0.784 \\
new\_year & 0.783 \\
rosh\_hashanah & 0.749 \\
\hline\end{tabular}\end{subtable}\begin{subtable}{.5\textwidth}\centering\subcaption{$c=\texttt{month}$}\begin{tabular}{ | t | c |}\hline
word & projection\\ \hline
august & 0.988 \\
april & 0.987 \\
october & 0.985 \\
february & 0.983 \\
november & 0.980 \\
\hline\end{tabular}\end{subtable}\vspace{5ex}

\begin{subtable}{.5\textwidth}\centering\subcaption{$c=\texttt{animal}$}\begin{tabular}{ | t | c |}\hline
word & projection\\ \hline
horses & 0.806 \\
moose & 0.784 \\
elk & 0.783 \\
raccoon & 0.763 \\
goats & 0.762 \\
\hline\end{tabular}\end{subtable}\begin{subtable}{.5\textwidth}\centering\subcaption{$c=\texttt{asian\_city}$}\begin{tabular}{ | t | c |}\hline
word & projection\\ \hline
taipei & 0.837 \\
taichung & 0.819 \\
kaohsiung & 0.818 \\
osaka & 0.806 \\
tianjin & 0.765 \\
\hline\end{tabular}\end{subtable}


